Monolith Development History for Microservices Identification: a Comparative Analysis

Recent research has proposed different approaches on the automated identification of candidate microservices on monolith systems, which vary on the monolith representation, similarity criteria, and quality metrics used. On the other hand, they are generally limited in the number of codebases and decompositions evaluated, and few comparisons between approaches exist. Considering the emerging trend in software engineering in techniques based on the analysis of codebases' evolution, we compare a representation based on the monolith code structure, in particular the sequences of accesses to domain entities, with representations based on the monolith development history (file changes and changes authorship). From the analysis on a total of 468k decompositions of 28 codebases, using five quality metrics that evaluate modularity, minimization of the number of transactions per functionality, and reduction of teams and communication, we conclude that the best decompositions on each metric were made by combining data from the sequences of accesses and the development history representations. We also found that the changes authorship representation of codebases with many authors achieves comparable or better results than the sequence of accesses representation of codebases with few authors with respect to minimization of the number of transactions per functionality and the reduction of teams.

==> arXiv - Monolith Development History for Microservices Identification_ a Comparative Analysis/evaluation.tex <==
\hypertarget{approach}{%
\subsection{Approach}\label{approach}}

The research goal, as stated in the introduction, is the
following:

\textbf{How do monolith microservices identification approaches that use the monolith code evolution representation perform when compared with approaches that use the monolith functionalities sequences of accesses representation?}

To address this research question, we generate a large set of
decompositions and analyse how the decomposition qualities vary
depending on different monolith representations and similarity measures.

Whenever we create a decomposition, we choose the weights to attribute
to our similarity measures. If we choose 0 as the weight for the commit
and the author similarity, then the decomposition is created using only
data from the sequences of accesses representation. On the other hand,
if we choose 0 as the weight for all four sequences of accesses measures
(access, read, write, sequence), then the decomposition is created using
only data from the development history based representations. In the
remaining combinations, the decompositions are created with data from
both sources. By filtering the results of all generated decompositions,
we can obtain five distinct groups of decompositions based on the
weights used to create them: only data from the file changes
representation; only data from the changes authorship representation;
only data from the sequences of accesses representation; only data from
the file changes representation and changes authorship; data from all
representations. This allows us to then compare the groups' quality
metrics and draw conclusions.

The comparisons will first be made by evaluating the median and the
dispersion of each quality metric in each of these five groups, which
gives us an overview of how, on average, each representation behaves. We
also evaluate the median values of the metrics in the case of the best
decompositions - that is, the decomposition of each codebase with the
best value for each metric. This gives us a different perspective by
focusing on which group performs best when the ideal weights for the
similarity measures are found. Finally, we assess if our findings hold
when we compare codebases with more commits and authors than the mean
with codebases with less commits and authors than the mean.

The comparisons are, initially, done visually through the analysis of
boxplots. Whenever it's not visually obvious that there is a large
difference between groups, and considering that there are different
amounts of decompositions in each group and the quality metric values
don't follow a normal distribution, we use a Welch T-test with the
following hypotheses:

\begin{itemize}
\tightlist
\item
  \(H_0\) - There are no significant differences between the mean
  \$\{QUALITY METRIC\} of \$\{GROUP\} decompositions and \$\{OTHER
  GROUP\}.
\item
  \(H_1\) - The mean \$\{QUALITY METRIC\} of \$\{GROUP\} decompositions
  is greater than \$\{OTHER GROUP\}.
\end{itemize}

\hypertarget{codebases-and-decompositions-characterization}{%
\subsection{Codebases and decompositions
characterization}\label{codebases-and-decompositions-characterization}}

In \cite{samuel22}, 121 codebases were chosen for evaluation. The
codebases were selected from GitHub, using the following procedure:

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  Get all GitHub repositories that list the Spring Data JPA library as a
  dependency;
\item
  Filter out repositories that did not contain at least 5 files whose
  name ended in \texttt{Controller.java}, and at least 5 files whose
  name did not contain \texttt{Dao} or \texttt{Repository}.
\item
  The remaining repositories were ordered by the number of GitHub stars,
  and 118 codebases were manually selected. Repositories from lessons or
  tutorials, and repositories that did not use just Spring Data JPA were
  disregarded.
\end{enumerate}

From this list, we selected 28 codebases by choosing those with at least
100 commits, and at least 2 authors. The codebases under study have a
mean commit count of 3080.8 with a standard deviation of 7604.5 (median
of 472), and a mean author count of 18.7, with a standard deviation of
30.1 (median of 6.5). This shows that we are only considering projects
with an actual development history, and not toy-like or quickly
abandoned projects.
% Information on the codebases names, their
% repositories, and cloned hash can be found on Mono2Micro's
% repository\footnote{\href{https://github.com/socialsoftware/mono2micro/blob/joao-commit-complexity/collectors/commit-collection/resources/codebases.csv}{codebases.csv
%   @ mono2micro's github}}.

% \begin{figure}[H]

% {\centering \includegraphics[width=\linewidth]{images/codebases-features-1} 

% }

% \caption{Plots showcasing some relationships of codebases' features: commit, authors, entities, and functionalities.}\label{fig:codebases-features}
% \end{figure}



For each codebase, we create decompositions with 3 to 10 clusters,
according to the number of entities it contains:
\(3 \leq n\_entities < 10 =\) 3 clusters; \(10 < n\_entities < 20 =\) 3,
4, and 5 clusters; \(n\_entities \geq 20 =\) 3 to 10 clusters. For each
number of clusters, we generate decompositions with varying weights on
the six measures: from 0 to 100, with increments of 10. The distribution
of the number of generated decompositions can be found in Table
\ref{tab:decompositions-characteristics}.

\begin{table}[H]

\caption{\label{tab:decompositions-characteristics}The number of generated decompositions across all codebases.}
\centering
\begin{tabular}[t]{llrr}
\toprule
\#Entities & \#Clusters & \#Codebases & \#Decompositions\\
\midrule
3 to 9 & 3 & 4 & 11982\\
10 to 19 & 3 to 5 & 8 & 72073\\
20+ & 3 to 10 & 16 & 384384\\
\midrule
\textbf{Total} & \textbf{} & \textbf{28} & \textbf{468439}\\
\bottomrule
\end{tabular}
\end{table}

\hypertarget{comparison-of-representations}{%
\subsection{Comparison of
representations}\label{comparison-of-representations}}

When evaluating the quality metrics of all decompositions of each
representation, we found that the development history representation
showed better results when it comes to cohesion than the sequence of
accesses, and the sequence of accesses, despite containing no data
regarding changes authorship, still performs well with regards to the
\emph{tsr}. For the coupling, complexity, and combined metrics, the
sequence of accesses representation often generated better
decompositions than the remaining representations.

Having concluded this, we now turn our analysis to the best
decompositions of each codebase. If we group all decompositions by
codebase and by number of clusters, and identify the minimum uniform
complexity decompositions in each group, we find that 92.95\(\%\) of the
best decompositions in terms of complexity were made by combining data
from the development history representations with the sequences of
accesses. Furthermore, 80.77\(\%\) of the best decompositions in terms
of cohesion, 95.51\(\%\) of the best decompositions in terms of
coupling, 95.51\(\%\) of the best decompositions in terms of \emph{tsr}
and 91.67\(\%\) of the best decompositions in terms of combined were
also obtained by this combination of representations. This finding,
together with the overview of the previous subsections, suggests that
the vast majority of weights combinations yield worse results than
considering just data from the sequences of accesses; but, if the right
combination is found, the results can be improved in almost all cases.

\begin{figure*}

{\centering \subfloat[Uniform complexity\label{fig:best-decompositions-compare-1}]{\includegraphics[width=0.3\linewidth]{images/best-decompositions-compare-1} }\subfloat[Cohesion\label{fig:best-decompositions-compare-2}]{\includegraphics[width=0.3\linewidth]{images/best-decompositions-compare-2} }\subfloat[Coupling\label{fig:best-decompositions-compare-3}]{\includegraphics[width=0.3\linewidth]{images/best-decompositions-compare-3} }\newline\subfloat[Team size reduction ratio\label{fig:best-decompositions-compare-4}]{\includegraphics[width=0.3\linewidth]{images/best-decompositions-compare-4} }\subfloat[Performance\label{fig:best-decompositions-compare-5}]{\includegraphics[width=0.3\linewidth]{images/best-decompositions-compare-5} }\subfloat[Legend\label{fig:best-decompositions-compare-6}]{\includegraphics[width=0.3\linewidth]{images/best-decompositions-compare-6} }

}

\caption{Grouping the decompositions by codebase and by number of clusters, and selecting the best decomposition in each group and each metric, highlights a difference between the representations and provides a different perspective on the results.}\label{fig:best-decompositions-compare}
\end{figure*}

Visually comparing the boxplots of the best decompositions of each
codebase, for each metric and for each monolith representation (Figure
\ref{fig:best-decompositions-compare}) shows that decompositions made
with the development history and the sequences of accesses
representations, simultaneously, display the best values in all metrics.
Statistical tests allow us to state with confidence that this is true
for uniform complexity, cohesion, coupling, and combined. This goes
against the conclusions drawn when considering all decompositions,
confirming our previous suggestion. For the case of \emph{tsr}, we
cannot say with confidence that this representation is better than just
the development history or the authorship, highlighting the poorer
performance that the sequence of accesses has in this metric.

\hypertarget{large-vs-small-codebases}{%
\subsection{Large vs small codebases}\label{large-vs-small-codebases}}

In our study so far, we made no distinction between small and large
codebases. But, there are 3 codebases with more commits than the mean
plus one standard deviation, which we call ``large in the number of
commits''. The remaining codebases are called ``small in the number of
commits''. A similar classification is made for the number of authors of
each codebase. Considering the increased information available from the
development history in these large codebases, we asked ourselves if
their development history based representations perform differently than
the representations of small codebases. To test this hypothesis, we
gathered the best decompositions of each representation for each metric,
and compare the best decompositions of large codebases in the number of
commits with small codebases in the number of commits, as well as large
codebases in the number of authors with small codebases in the number of
authors. Box plots with these comparisons can be found in Figure~\ref{fig:large-small-codebases-compare}.

We can say with statistical significance that the median uniform
complexity of small codebases in the number of authors is greater than
that of large codebases in the number of authors, when comparing the
authorship representation for both cases (p-value: 0). We can also state
that there are no significant differences between the median uniform
complexity of the authorship representation in large codebases to the
median uniform complexity of the sequences representation in small
codebases, whereas there is a difference if we compare these two
representations in small codebases. This is a surprising result, as it
suggests the effectiveness of the authorship representation, when
compared with sequences, if more authors are present.

We can also say that the \emph{tsr} of the smaller codebases in the
number of authors is greater than the large ones in all representations.
Statistical tests reveal that there are no significant differences
between the authorship, development history, and the combined
development history and sequences representations, highlighting the
effect that the changes authorship data has in these representations.
Similarly to the uniform complexity, the development history based
representations of large codebases perform better than the sequence of
accesses of small codebases, whereas they perform worse in the case of
smaller codebases. Regarding coupling, the obtained values in the files
and authorship representations are very similar for both categories of
codebases, visually and with statistical significance, but the smaller
codebases display worse values in the development history, sequences,
and the development history and sequences representations. The good
performance of the larger codebases in the number of authors explains
the improvement of the combined metric, as the representations of
smaller codebases have statistically significant greater median values
than the large codebases. The only metric where the large codebases in
the number of authors do not display better results than the smaller
codebases is cohesion.

Large codebases in the number of commits display improved \emph{tsr}
median values across all representations, when compared with small
codebases in the number of commits. In the case of uniform complexity
and, consequently, combined, better results are obtained for the files
representation of large codebases (when compared with the files
representation of small codebases) only if we discard one of the large
codebases (Irida) that does not behave like the others. We find that the
modularity is neither improved nor worsened when we evaluate codebases
with more commits. In the case of cohesion, the smaller codebases in the
number of commits are similar to the large, and other than the
authorship representation, we do not find statistically significant
differences between their medians. For coupling, cannot confidently
state that the larger codebases have greater median than the smaller.
For the combined metric, we cannot state that the smaller codebases
display larger values in any representations, which means that overall,
the quality of codebases with more commits is comparable to the quality
of codebases with less commits.

Finally, we can state that just like in the previous analysis of the
best decompositions, the best results are obtained when combining the
development history with sequences of accesses, in all quality metrics -
both for large and small codebases in the number of commits and authors.

% \begin{figure*}

% {\centering \subfloat[Uniform complexity\label{fig:large-small-codebases-compare-1}]{\includegraphics[width=0.3\linewidth]{images/large-small-codebases-compare-1} }\subfloat[Cohesion\label{fig:large-small-codebases-compare-2}]{\includegraphics[width=0.3\linewidth]{images/large-small-codebases-compare-2} }\subfloat[Coupling\label{fig:large-small-codebases-compare-3}]{\includegraphics[width=0.3\linewidth]{images/large-small-codebases-compare-3} }\newline\subfloat[tsr\label{fig:large-small-codebases-compare-4}]{\includegraphics[width=0.3\linewidth]{images/large-small-codebases-compare-4} }\subfloat[Combined\label{fig:large-small-codebases-compare-5}]{\includegraphics[width=0.3\linewidth]{images/large-small-codebases-compare-5} }\subfloat[Legend\label{fig:large-small-codebases-compare-6}]{\includegraphics[width=0.3\linewidth]{images/large-small-codebases-compare-6} }

% }

% \caption{Comparison between the best decompositions of each representation. Different results are obtained when we compare large with small codebases.}\label{fig:large-small-codebases-compare}
% \end{figure*}


\begin{figure*}

{\centering \subfloat[Uniform complexity\label{fig:large-small-codebases-compare-1}]{\includegraphics[width=0.46\linewidth]{images/large-small-codebases-compare-1} }\subfloat[Cohesion\label{fig:large-small-codebases-compare-2}]{\includegraphics[width=0.46\linewidth]{images/large-small-codebases-compare-2} }\newline\subfloat[Coupling\label{fig:large-small-codebases-compare-3}]{\includegraphics[width=0.46\linewidth]{images/large-small-codebases-compare-3} }\subfloat[tsr\label{fig:large-small-codebases-compare-4}]{\includegraphics[width=0.46\linewidth]{images/large-small-codebases-compare-4}}\newline\subfloat[Combined\label{fig:large-small-codebases-compare-5}]{\includegraphics[width=0.46\linewidth]{images/large-small-codebases-compare-5} }\subfloat[Legend\label{fig:large-small-codebases-compare-6}]{\includegraphics[width=0.46\linewidth]{images/large-small-codebases-compare-6} }

}

\caption{Comparison between the best decompositions of each representation. Different results are obtained when we compare large with small codebases.}\label{fig:large-small-codebases-compare}
\end{figure*}


% To answer our research question, we can conclude that the authorship
% representation for large codebases provides similar results to the
% sequences of accesses. This allows the usage of a collection technique
% that is easier to apply, as it is independent of the language or
% framework chosen for the monolith.



\subsection{Discussion}

We were able to properly compare the various representations in previous
sections, through visual analysis and statistical analysis. The median
quality metrics values across all codebases and clusters provided us
with an overview of the most common scenario. But this is a limited
view, as it does not fully represent what happens if an ideal
decomposition is found. To fix that, we also analyzed the best
decompositions of each metric and representation, where often different
results were obtained. Additionally, we often could not find significant
differences between the development history based representations, so we
separated the best decompositions according to the number of commits and
authors of their codebases, which gave us better insights in some
situations.

This whole analysis provided us with several conclusions that allow us
to answer the research question, focused around how the
sequences of accesses representation compares with development history
based representations:

\begin{itemize}
\item
  On average, the sequence of accesses representation is better in the
  case of complexity and coupling. For cohesion, no significant
  differences were found between representations, with the exception of
  the changes authorship representation, which performs worse than all
  others. On the other hand, representations with change authorship
  data, like the changes authorship, development history, and
  development history and sequences, perform better than the sequence of
  accesses for \textit{tsr}, although we have to highlight the still
  acceptable performance of the latter. These trade-offs are captured by
  the combined metric and confirmed through statistical tests, as we
  cannot state that any representation is better than the others at any
  number of clusters.
\item
  When looking at the best decompositions, the combined development
  history and sequence of accesses representation yielded the best
  values for all metrics. A notable exception is in the \textit{tsr} metric,
  where we could not state with statistical significance that this
  representation is better than the development history representation.
  Nevertheless, these conclusions give support to the notion that the
  presence of more data from different sources improves results.
  However, considering that this does not happen when looking at the
  vast majority of decompositions, it means that obtaining good results
  when using data from the development history is very dependent on
  choosing the ideal weights when creating the decomposition.
\item
  Through the comparison between large and small codebases in the number
  of commits and/or authors, we cannot state that the complexity of the
  changes authorship representation of large codebases in the number of
  authors is higher than the sequences of accesses representation of
  small codebases in the number of authors. Regarding cohesion and
  coupling, we found that the presence of more commits or authors does
  not improve results. On the other hand, more commits or authors does
  significantly improve the \textit{tsr} values, as any representation of
  larger codebases has a better median than the sequences of accesses
  representation of smaller codebases.
\end{itemize}

\hypertarget{threats-to-validity}{%
\subsection{Threats to validity}\label{threats-to-validity}}

Out of all decompositions, we find that \(0.37\%\) were made exclusively
with data from the development history, and \(9.52\%\) exclusively with
data from the sequences of accesses. The remaining \(90.11\%\) were made
with combined data. This is a consequence of using four measures related
to the sequences of accesses, but only two related to the development
history. To ensure this does not affect our findings, we opted to use a
statistical test that performs well even comparing groups with different
sample sizes, and do not rely only on boxplots to draw conclusions.
Additionally, note that these differences only applied for the first
analysis, where we consider to all the decompositions, which was rather
inconclusive. For all the other analyses, the best decompositions were
chosen and so, we have only one decomposition per representation and
number of clusters.

Not all repositories have a clean and linear history, with some
presenting many branches, refactors, and merges. This affects the
detection and processing of deletes and renames, which makes development
history based decompositions less efficient. Nevertheless, we obtained
good results for the development history representations.

We found that sometimes, files presented an \texttt{ADD} or
\texttt{MODIFY} change event after a \texttt{DELETE} event. In some
situations, this means we could be considering two distinct files as the
same one, if they happened to have the same filename and one of them was
deleted before the other was added. However, in all cases we found, the
files still existed in the latest repository snapshot and did correspond
to the same file that was deleted. Considering that this situation is
unlikely, and the existence of a \texttt{DELETE} event after an
\texttt{ADD} or \texttt{MODIFY} change event usually occurs due to
merges, we opted to still consider these files in our analysis, and we
don't discard them.

Our data collection approach was to gather data about all \texttt{.java}
files across all commits, and then discard non domain entities files
only in the decomposition phase. An alternative would be to filter all
commits and select those where only domain entities were changed. Our
approach is richer, as we have more data available and are not deleting
potentially useful relationships between files.

We adapted the logical coupling and the contributor coupling measures
from \cite{mazlami_extraction_2017}, by considering a fraction rather
than an absolute value. This was made to facilitate the integration of
other measures without much experimentation on the ideal weights that
would be required if absolute values were considered.

